Generative Concatenative Nets Jointly Learn to Write and Classify Reviews

A recommender system's basic task is to estimate how users will respond to unseen items. This is typically modeled in terms of how a user might rate a product, but here we aim to extend such approaches to model how a user would write about the product. To do so, we design a character-level Recurrent Neural Network (RNN) that generates personalized product reviews. The network convincingly learns styles and opinions of nearly 1000 distinct authors, using a large corpus of reviews from BeerAdvocate.com. It also tailors reviews to describe specific items, categories, and star ratings. Using a simple input replication strategy, the Generative Concatenative Network (GCN) preserves the signal of static auxiliary inputs across wide sequence intervals. Without any additional training, the generative model can classify reviews, identifying the author of the review, the product category, and the sentiment (rating), with remarkable accuracy. Our evaluation shows the GCN captures complex dynamics in text, such as the effect of negation, misspellings, slang, and large vocabularies gracefully absent any machinery explicitly dedicated to the purpose.

==> sections/acknowledgments.tex <==
Zachary C. Lipton's research is funded by the UCSD Division of Biomedical Informatics,
via NIH/NLM training grant T15LM011271.
Sharad Vikram's research is supported in part by NSF grant CNS-1446912.
We would like to thank Professor Charles Elkan for his mentorship.
We gratefully acknowledge the NVIDIA Corporation, whose hardware donation program furnished us with a Tesla K40 GPU, making our research possible.

==> sections/category-tracking.tex <==
Here we show several representative examples demonstrating the ability of the generative concatenative network (run in reverse) to recognize the category of the beer at the precise point in the sentence when it becomes clear. At first the probabilities are all close to $.2$ reflecting the uniform prior. By the end of the sentences the distribution conditioned on the input is considerably less entropic.

\begin{figure}[ht]
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/smoky-porter.png}
  \caption{``This beer has a smoky taste.''}
  
  \label{fig:smoky-porter}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/pours-black.png}
  \caption{``Pours a black color.''}
  \label{fig:pours-black}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/nice-dark-black-stout.png}
  \caption{``Very nice dark black stout.''}
  \label{fig:nice-dark-black}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/pours-amber.png}
  \caption{``Pours an amber color.''}
  \label{fig:pours-amber}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/love-strong-hoppy.png}
  \caption{``Love the strong hoppy flavor.''}
  \label{fig:strong-hoppy}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/bitter-ipa.png}
  \caption{``This beer is bitter.''}
  \label{fig:bitter-ipa}
\end{subfigure}
\caption{We plot the probabilities of the $5$ beer categories after each character in the sentence is encountered.}
\label{fig:cat-track}
\vspace{-10pt}
\end{figure} 

==> sections/encode-concat.tex <==
In this paper, we introduced and demonstrated the efficacy of a simple technique for incorporating auxiliary information $\boldsymbol{x_{aux}}$ in a generative RNN by concatenating it with with the character representation  $\boldsymbol{x}_{char}^{(t)}$ at each sequence step.
However, sometimes we don't simply want to generate given a representation $\boldsymbol{x_{aux}}$, but to learn a representation of $\boldsymbol{x_{aux}}$.
For example, to generate a character-level caption given an image, 
we might want to jointly learn a convolutional neural network to encode the image, and a generative RNN to output a caption.

To accomplish this task at the character level, 
we propose the following network architecture
and hypothesize that is will provide 
the benefits of learning an encoding
while preserving our ability to generate long passages 
at the character level. 
At train time the $\boldsymbol{x_{aux}}$ 
is fed to an encoder, 
whose output is then passed as auxiliary information to a concatenated input network. 
At prediction time, for any input, 
the encoding is calculated once, 
after which the inference problem 
is identical to that of our demonstrated concatenated input network.


\begin{figure}[ht]
  \begin{center}
% 	\vspace{-20pt}
	\includegraphics[width=1.0\textwidth]{img/encode-concat.png}
%     \vspace{-25pt}
  \end{center}
  \caption{Generative model with input replication. We train the network to produce a \emph{5 star} review by concatenating the rating with the one-hot representation of each character.}
  \label{fig:encode-catnet}
\end{figure} 

==> sections/generate-item.tex <==
In the following examples, we generate reviews conditioned on the item category. We show one example each for American IPA, American Adjunct Lager, Russian Imperial Stout, American Porter, and Fruit/Vegetable Beer. All reviews in this section are generated with a temperature of $.5$

\subsection{American IPA}
\begin{displayquote}
$<$STR$>$Pours a transparent copper with a nice creamy off-white head that retains well and leaves behind a nice lace.	S: Mild aroma of citrus and pine hops. The smell is not super pleasing. T: The body isn't overly abused by the orange peel flavors. It is a solid IPA that is followed by a mouthfeel with a huge rich malt background that is quite prevelent. The finish is slightly bitter on the tongue, and the malt is slightly dry by the end. A touch of sweet malts in the background.	M: Great carbonation and a light moderate carbonation feel. Flavors are very pleasant nicely balanced by the hops and resins.	D: This is an easy drinking IPA and I would definitely like to try it again for what it is anyway.	Overall: This is a well crafted beer. It is a great example of an IPA, I would definitely have another one of these and I will be getting another can in the bottle and like to see it more in the can in some time.$<$EOS$>$
\end{displayquote}
    
\subsection{American Adjunct Lager}
\begin{displayquote}
$<$STR$>$A - Poured a dark yellow color with a white head that leaves lacing behind	S - Lightest aroma, some corn with a slight hop presence. It has a fairly strong aroma of corn and yeast. The taste is slightly sweet and crisp, corn and a light hop presence. The finish is moderately bitter with a slight sweetness. Finishes sweet and clean with a light crisp finish. Not much more to say. This would be a good one to have when ice cold, and I'd rather have a Coors Light.$<$EOS$>$
\end{displayquote}
    
\subsection{Russian Imperial Stout}
\begin{displayquote}
$<$STR$>$Thanks to Buttlepoptu for the chance to try this one. Got this bottle from a 12 oz. bottle in a tasting glass. A- Pours a deep black color with a miniscule head that dissipates quickly. No lacing to speak of either. S- Nice bitter chocolate nose. Lots of chocolate, coffee, roasted coffee, and a little chocolate. T- The dark roasted malts provide a sweet finish, and in the most refreshing taste and the bitterness of this one is a little subdued. M: Thick and rich, like syrup. Slick and creamy. Sits right away and it lasts for just a little D: What a world class RIS. While I love all the world of beers that I've tried in the past, this is very drinkable. I think it could be a little much for sure. Still a good beer for sure. This one is worth the wait. While it is not a beer I could drink a few of without getting a little difficult to drink and finish the whole bottle.
$<$EOS$>$
\end{displayquote}
    
\subsection{American Porter}
\begin{displayquote}
$<$STR$>$ 
Served a beautiful black with a mocha head that started about 1/1 inch thick and left lots of lacing. The smell was sweet and roasty with some vanilla and a hint of chocolate. The taste was primarily that of smoky chocolate and some chocolate and barrel character. It had a light mouthfeel with a crisp carbonation. Overall this was a very good beer. I was more interested in pouring this one from a bottle though it is a very good brew (that a must have again). I have another one on tap and it was my ease of time.	Overall: A big thanks to Richmond for the chance to try this one. I've enjoyed other porters to be but this is definitely a porter.
$<$EOS$>$
\end{displayquote}
    
\subsection{Fruit/Vegetable Beer}
\begin{displayquote}
$<$STR$>$On tap at the brewpub. A nice dark red color with a nice head that left a lot of lace on the glass. Aroma is of raspberries and chocolate. Not much depth to speak of despite consisting of raspberries. The bourbon is pretty subtle as well. I really don't know that I find a flavor this beer tastes like. I would prefer a little more carbonization to come through. It's pretty drinkable, but I wouldn't mind if this beer was available.
$<$EOS$>$
\end{displayquote}
    

==> sections/generate-star.tex <==
Below, we show examples of the generative concatenative network's ability to generate decidedly positive reviews when conditioned on high star ratings and decidedly negative reviews when conditioned on low ratings. Because the star rating is simply a scalar input to the network, we can also generate reviews conditioned on the more extreme $0$ star and $10$ star ratings, even though neither truly exist in the dataset. We present examples of reviews generated by the model and conditioned upon $0$, $1$, $5$, and $10$ star ratings. For each we show an example each for three settings of the temperature (.1, .5, 1.0).

\subsection{0 Star Reviews}
The following full reviews are generated conditioned on a $0$ star rating for varying settings of the temperature.

With a temperature of $.1$

\begin{displayquote}
$<$STR$>$Pours a clear amber with a thin white head that dissipates quickly. Smell is of caramel malts and some hops. Taste is a little sweet and malty. The mouthfeel is thin and watery. This is a very disappointing beer. I would not buy this again.$<$EOS$>$
\end{displayquote}

With a temperature of $.5$:

\begin{displayquote}
$<$STR$>$This is an old bottle of a premium beer. This was a bad batch.	Pours a color that is black. The head is a small bubbling of bubbles with a thick ring and leaves some nice lacing.	The aroma is a strong metallic twang and some light chocolate notes. The smell is of cocoa and coffee. While the aroma is an astringent blast of chocolate and coffee on the nose. The taste is also filled with a very strong alcohol flavor. It tastes like a bad barleywine. The flavors are very strong, and the malt and dark fruits take over the flavor. The mouthfeel is thin and watery. The drinkability is not good.$<$EOS$>$
\end{displayquote}

With a temperature of $1.0$

\begin{displayquote}
$<$STR$>$The color is a rice golden the body with fizzy yellow carbonation (which is unpleasant). No lacing, which suffers from half an inch. Anyway: horrible, suck, surprise, and unpleasant. I below a dubbel, but the honey seems a bit distracting. Thin almost taste of baked bread, caramel malt and almonds...very sickly without much addition into the bottom of perhaps in my mouth. This beer conversely, but then again my rear sourness really kicked up the malt and lies.	Mouthfeel was fine.	I was difficult to finish this fixe a year and thank Guinness at a party beer. I say this is one very watered down beer.$<$EOS$>$
\end{displayquote}


\subsection{1 Star Reviews}
With a temperature of $0.1$
\begin{displayquote}
$<$STR$>$Pours a clear amber with a thin white head. Smell is of sweet malt, and a hint of caramel. Taste is also sweet and malty with a slight hop bitterness and a slight bitterness. Mouthfeel is medium bodied with a smooth and creamy mouthfeel. This is a beer that I will probably not go out of my way for any time soon.$<$EOS$>$
\end{displayquote}


With a temperature of $0.5$
\begin{displayquote}
$<$STR$>$A: Pale yellow color with a small white head.	S: Spicy and citrusy.	T: Sweet and sour fruit with a bit of a metallic taste at the end.	M: Light, sticky, and syrupy.	D: Somewhat tasty, but the alcohol does not have a lot of complexity to the beer. I would not buy this again.$<$EOS$>$
\end{displayquote}

With a temperature of $1.0$
\begin{displayquote}
$<$STR$>$This beer was gone alright. It did not go away. It's all about the booze, but it seems a rather peppery, aggressive, heavy, smelling (at times) for something better. No where near as big as I'd like. Artificially. You would love this beer... even a sipper. If kolsh were an oddball sourness, I'd swear this one would win. I haven't been afraid of my fridge selection for less money.$<$EOS$>$
\end{displayquote}


\subsection{5 Star Reviews}
With a temperature of $0.1$
\begin{displayquote}
$<$STR$>$Poured from a 12 oz. bottle into a pint glass.            Appearance: Pours a clear golden color with a thick frothy white head that slowly fades to lacing. The aroma is great. It has a sweet caramel malt aroma with a slight hop aroma. The taste is a little sweet with a slight hop bitterness that lingers in the aftertaste. The mouthfeel is medium bodied with a good amount of carbonation. This is a very drinkable beer. I would have no problem drinking a few of these in a sitting. I would definitely drink this again in the future.$<$EOS$>$
\end{displayquote}

With a temperature of $0.5$
\begin{displayquote}
$<$STR$>$A - Poured a midnight black with a thick frothy tan head that left lacing on the glass.           S- Smell is a wonderful virtual malt aroma with a touch of coffee and chocolate. Taste is chocolate and coffee with a hint of chocolate and coffee. Its a little thin for a witbier at all.           M- This beer has a medium mouthfeel with a slight amount of carbonation.             D - Very drinkable beer. I could drink this all night long. I will definitely be buying a few more in the cellar.$<$EOS$>$
\end{displayquote}

With a temperature of $1.0$
\begin{displayquote}
$<$STR$>$First off, I have batch whose pure vertical esopetime trade! The forgot "Homaching copper" IPA would be a popular beer fixed in Pounds VE! Poured into Duvel tulip.          APV of caramel with a small light tan head that cakes off on the glass now and lays down to a thin layer of residence that leaves behind dots of lace as it settles. Several left behind with remarkable introducing curtains.                Aroma is enveloping massive but incredibly were redolent -- refreshing. Juicy Belgian yeast esters - bursts of lime, lemon pith, etc... all right up front. Spiciness is in a glorious essence. Really man's Belgian pale and wild yeast funk too. Basically the taste's aroma is mostly grapefruit juice and vegetably accents. hints of oak, cranberries and light hints of yeast funk. A faint funkiness in there as well, with all malts. And smooth and a bit muddy too.               Finish is fresh and both easy to glass, you know the glass who dies on that sweetness itself, but you still think you what effect you get - it makes the least busy-love color? Stone has perfect!    Mouthfeel is smooth and clean with an earthy smoothness that lack the nice sharp bite of the malt and certain to exquisitely surface from the malt. Exceptional imperial stout. Low to drinkability, in an awesome winter warmer, especially when a bit of age doesn't work for me. A 20\% beer is only great by my someone worry but a beer that would go well with something along with my friend. Nicely done in any mark. Superb.$<$EOS$>$
\end{displayquote}


\subsection{10 Star Reviews}

With a temperature of $0.1$
\begin{displayquote}
$<$STR$>$Poured from a 12 oz. bottle into a pint glass.            Appearance: Pours a dark brown color with a thick tan head that lasts forever and leaves a nice lacing on the glass. The aroma is of chocolate, coffee, chocolate, and a hint of chocolate. The taste is a nice blend of coffee, chocolate, and coffee. The mouthfeel is smooth and creamy with a nice creamy feel to it. This is a very good beer that I would definitely have again. I would love to have this again and again. I wish I had more of this stuff and see how this is the best beer I've ever had. I could drink this all day and enjoy it all the time. I could drink this all day and drink all day. I could drink this all day and drink all day and savor the other three of these and this is a staple in my fridge.$<$EOS$>$
\end{displayquote} 

With a temperature of $0.5$
\begin{displayquote}
$<$STR$>$A- Amber brown with a small white head that has decent retention and leaves a nice lacing on the glass. Aroma is strong of citrus hops and a mild sweet malt aroma. The taste is so smooth and crisp tasting with the hops throughout the taste. The malt is more citrus than I expect to be sure this is a hop bomb with the alcohol in this beer that makes it easy to drink and smooth. The alcohol is noticeable and delicious. This is a great beer, and a great take on the style and one of the best in the world. I could drink this all night. I guess the alcohol is evident in the flavor and the flavors are bright and crisp and drinks smoother and is so easy to drink. I wish I had more! This is the best beer that I've ever had in awhile. I would definitely order it again and again.$<$EOS$>$
\end{displayquote}

With a temperature of $1.0$
\begin{displayquote}
$<$STR$>$A: Pours vibrant amber with a nice, hugs foamy head. Awesome light brown sheen that looks like it.              successful excellent! Want down thoroughly IPA indeed. Soft with pine and lime juice (since you sat down!) come through at most. Also kicking bach down from something dampeness.             Take through the enjoyment of this is wonderful for sure. Delicious. Is this rank? Now that it full body's imperessively. Espresso-strock, this beer is that fantastic. You will nip sip that OK. I drink one beer yet! I can't remember the 2008 version I might even paybe local!$<$EOS$>$
\end{displayquote}


==> sections/latent-factors.tex <==
While experiments with one-hot representations
and dense subsets of the reviewer community
provide a proof of concept that our techniques 
can synthesize personalized reviews,
such an approach cannot scale to the enormous real-life datasets.
First, with 1024 LSTM nodes in each layer, 
each user requires an additional 4096 parameters.
This presents computational problems as the full weight matrices could not be stored in main memory as the number of users grows large.
Second, to fit so many weights without overfitting we need many reviews for each user.
The vast majority of users of most websites have not written hundreds of reviews.

For many sites, such as Amazon, 
many users have written not reviews, 
but have provided other information,
such as ratings and purchase history.
Thus we seek to generate reviews conditioned on latent representations learned from the task of rating prediction.
Such representations offer us a mechasnism for generating personalized reviews
even for users that never appear in the training set.

The latent factors are learned by training a simple regression model 
to predict the rating assigned to a given item by a given user.
Each user $u$ is modeled by a latent vector $\gamma_u \in \mathbbm{R}^k$ while each item $i$ is similarly represented with a latent vector $\gamma_i \in \mathbbm{R}^k$
Additionally, each item and each user is a associated with a bias,
$\beta_i$ and $\beta_u$ respectively.
Thus the ratings model is given by
$$\hat{r} = \alpha + \beta_i +\beta_u + \gamma_i \cdot \gamma_u$$
Where the dot product between the user vector and item vector 
indicates their compatibility.
For this work we train latent factors of dimension 10 for users and items 
and evaluate the ability of the GCN to produce reviews with low perplexity using only this information.

==> sections/learning-curves.tex <==
For each task, we train two unsupervised character-level \emph{donor} RNNs 
so that we may harvest the weights for transplantation
into the concatenated input networks.
We train separate \emph{donor} networks for the two tasks (rating and category modeling) because each is trained on a different subset of the data (the beer set is selected for class balance among the $5$ categories and is thus smaller).
These networks are trained until convergence (\autoref{fig:charnet-learning}).
After transplantation, we train the concatenated input RNNs with high learning rates, to induce the weights for auxiliary
information to grow quickly. This results in
an initial spike in loss (to quick to be seen in \autoref{fig:charnet-learning-transplant}), after which the loss quickly decreases.

\begin{figure}[ht]
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=1\textwidth]{img/charnet-ratnet_learning.png}
\caption{Unsupervised rating network}
\label{fig:charratnet-learning}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=1\textwidth]{img/charnet-catnet_learning.png}
\caption{Unsupervised category network}
 \label{fig:charcatnet-learning}
\end{subfigure}
\caption{The learning curves for the unsupervised donor character RNNs
used for weight transplantation.}
\label{fig:charnet-learning}
\end{figure}

\begin{figure}[ht]
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=1\textwidth]{img/ratnet-learning_curve.png}
\caption{Rating network after transplantation}
\label{fig:ratnet-learning}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=1\textwidth]{img/catnet-learning_curve.png}
\caption{Category network after transplantation}
 \label{fig:catnet-learning-transplant}
\end{subfigure}
\caption{The learning curves for rating and category networks after weight transplantation.}
\label{fig:charnet-learning-transplant}
\end{figure}

==> sections/negation.tex <==
The following charts present anecdotal evidence that the GCN is able to learn nonlinear dynamics. Here we show that the model can learn that ``not great" corresponds to a worse rating than ``great'' while ``not bad'' corresponds to better rating than ``bad''.

\begin{figure}[ht]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/great-endgraph.png}
  \caption{``This beer is great."}
  \label{fig:great}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/not-great-endgraph.png}
  \caption{``This beer is not great"}
  \label{fig:not-great}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/bad-endgraph.png}
  \caption{``This beer is bad."}
  \label{fig:bad}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/not-bad-endgraph.png}
  \caption{``This beer is not bad."}
  \label{fig:not-bad}
\end{subfigure}
\caption{We plot the likelihood given 
to a review by each rating. The network learns nonlinear dynamics of negation. ``Not" reduces the rating when applied to ``great" but increases the rating when applied to ``bad". }
\label{fig:negation-phrasegraph}
\vspace{-10pt}
\end{figure} 

==> sections/rating-endgraphs.tex <==
The following graphs show the likelihood of each sentence conditioned upon various settings of the rating. As expected, positive sentences are more likely given positive ratings while negative setences are more likely given negative ratings. Sentences indicating mixed sentiment tend to be most likely given appropriately lukewarm ratings.

\begin{figure}[ht]
\centering
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/mindblowing-endgraph.png}
  \caption{``Mindblowing experience."}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/watered-down-endgraph.png}
   \caption{``Tastes watered down."}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/best-worst-endgraph.png}
   \caption{``Not the best, not worst."}
\end{subfigure}
\caption{ Log likelihood of the review 
for many settings of the rating. 
This tends to be smooth and monotonic for unambiguous sentences, but peaks in the center for less extreme sentiments.}
\label{fig:endgraph}
\vspace{-10pt}
\end{figure} 

==> sections/sentiment-tracking.tex <==
As each character in a review is encountered, we can plot the rating (with a granularity of 100 evenly spaced settings between 1 star and 5) which gives the review highest likelihood. Thus we can tell not only the sentiment of the rating, but the precise word, and even character at which this sentiment became clear.

\begin{figure}[ht]
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/beast-beer.png}
  \caption{``Simply the beast offering in the category ever.''}
  \label{fig:the-beast}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/without-a-doubt.png}
  \caption{``Without a doubt one of the best 3 beers I've had the pleasure of trying.''}
  \label{fig:without-a-doubt}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/light-watery-skunky.png}
  \caption{``Light, watery, skunky, cheap.''}
  \label{fig:light-watery-skunky}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/worst-beers.png}
  \caption{``One of the worst beers I've ever had.'}
  \label{fig:worst-beers}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/nothing-bad.png}
  \caption{``There's absolutely nothing bad to be said about this beer.''}
  \label{fig:nothing-bad}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/no-flavor.png}
  \caption{``There's really no flavor to speak of here.'}
  \label{fig:no-flavor}
\end{subfigure}
\caption{We plot the argmax of the review's likelihood over many settings of the rating.}
\label{fig:sentiment-track}
\vspace{-10pt}
\end{figure} 
